Strong Completeness and the Finite Model Property for Bi-Intuitionistic Stable Tense Logics

Bi-Intuitionistic Stable Tense Logics (BIST Logics) are tense logics with a Kripke semantics where worlds in a frame are equipped with a pre-order as well as with an accessibility relation which is 'stable' with respect to this pre-order. BIST logics are extensions of a logic, BiSKt, which arose in the semantic context of hypergraphs, since a special case of the pre-order can represent the incidence structure of a hypergraph. In this paper we provide, for the first time, a Hilbert-style axiomatisation of BISKt and prove the strong completeness of BiSKt. We go on to prove strong completeness of a class of BIST logics obtained by extending BiSKt by formulas of a certain form. Moreover we show that the finite model property and the decidability hold for a class of BIST logics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{105}
\providecommand{\publicationstatus}{Sujata Ghosh and R. Ramanujam: M4M9\\
EPTCS 243, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.243.8}{10.4204/EPTCS.243.8}}
\pdfoutput=1

